Holographic Gravitational Anomaly in First and Second Order Hydrodynamics

We compute, in the framework of the fluid/gravity correspondence, the transport coefficients of a relativistic fluid affected by chiral and gauge-gravitational anomalies, including external electromagnetic fields. The computation is performed at first and second order in the hydrodynamical expansion. We use a 5-dim holographic model with pure gauge and mixed gauge-gravitational Chern-Simons terms in the action. We reproduce at first order previous results on the anomaly induced current of a magnetic field and a vortex in a relativistic fluid, and compute at second order the anomalous and non anomalous transport coefficients by using a Weyl covariant formalism. We find a dissipative and anomalous correction to the chiral magnetic conductivity due to the time dependence of the magnetic field. We also find a new contribution from the mixed gauge-gravitational anomaly to the shear waves dispersion relation. The role played by the chiral and gravitational anomalies in other transport coefficients is discussed.

==> kubo.tex <==

Actually the presence of $\tilde{\xi}_5$ must be captured by  a model in the probe limit. The very simple model of the Chapter \ref{cmecse} is enough to be used as a consistency check. In order to proceed we will work only with an axial gauge field switched on, so we just need to solve the equations (\ref{eq:probe_axial}) and follow the standard holographic procedure describe in previous chapters in order to obtain the retarded correlator, the final result is
{\small\begin{equation}
\langle \mathcal J^a \mathcal J^b\rangle=\left(
\begin{array}{cc}
 -\frac{i \omega }{g_A}+\omega^2 \frac{ \log 2}{2 g_A}-72  g_A  (k\kappa  \mu) ^2 (-1+\log 4) & -12 i k  \kappa   \mu +12 k \omega  \kappa  \mu \log 2 \\
 12 i k   \kappa   \mu -12 k \omega  \kappa  \mu \log 2 & -\frac{i \omega }{g_A}+\omega^2 \frac{ \log 2}{2 g_A}-72(k\kappa  \mu) ^2  g_A   (-1+\log 4)
\end{array}
\right).  \label{eq:jjsecorderMatrix}
\end{equation}}

In order to relate the fluid/gravity model with the one in Chapter \ref{cmecse} we have to do the following redefinitions
\begin{eqnarray}\nonumber
\kappa &\rightarrow & 24\pi G \kappa \qquad , \qquad r_+  \rightarrow  1  \,, \\
\nonumber g_A^2 &\rightarrow & 16\pi G \qquad \textrm{and} \qquad T \rightarrow \frac{1}{\pi} \,.
\end{eqnarray}
On the other hand, by using Eq.~(\ref{eq:xitilde5}) and after doing a linear expansion for $\bar{\mu}\ll 1$ we get
\begin{equation}
\tilde{\xi}_5= 12\kappa  \mu  \log 2  - \frac{\lambda  \mu }{\pi G r_+} \left(1 + 2 \log 2\right) +  \mathcal{O}(\bar{\mu}^3)\,.
\end{equation}
When we compate the $\kappa-$part of this result with the one obtained from the Kubo formulae~(\ref{eq:jjsecorder}) and (\ref{eq:jjsecorderMatrix}), both results agree. We can only compare the $\kappa$ contribution, as the correlator was computed in the probe limit where the backreaction of the gauge field on the background black hole is neglected and in consequence the effect of the gravitational anomaly is subleading.

